Predicting Information Pathways Across Online Communities

The problem of community-level information pathway prediction (CLIPP) aims at predicting the transmission trajectory of content across online communities. A successful solution to CLIPP holds significance as it facilitates the distribution of valuable information to a larger audience and prevents the proliferation of misinformation. Notably, solving CLIPP is non-trivial as inter-community relationships and influence are unknown, information spread is multi-modal, and new content and new communities appear over time. In this work, we address CLIPP by collecting large-scale, multi-modal datasets to examine the diffusion of online YouTube videos on Reddit. We analyze these datasets to construct community influence graphs (CIGs) and develop a novel dynamic graph framework, INPAC (Information Pathway Across Online Communities), which incorporates CIGs to capture the temporal variability and multi-modal nature of video propagation across communities. Experimental results in both warm-start and cold-start scenarios show that INPAC outperforms seven baselines in CLIPP.

==> src/bak.tex <==
\subsubsection{Global influence}
 
 Infer a subreddit-subreddit influence network. 
 
 \noindent \textbf{Input} A set of propagation sequences $\{\{(v_i, u_j, s_j, t_j)\}_{j=1}^N\}_{i=1}^{|V|}$
 

 \noindent \textbf{Output} A homogeneous weighted directed graph $G_S$ consisting of 
 
 \yiq{This task does not have ground-truth supervision signals. So I think we can write it in a discovery style}



%%% Prototypical Network %%%

 and channel names of the videos. Each video $v_i$ and channel $c_j$ are encoded into feature representations $\mathbf{v}_i, \mathbf{c}_j \in \mathbb{R}^{D}$, where $D$ is the dimension of the feature vector.
The video embeddings contain rich semantic features. Due to the parametric aspect of the model, it can be inefficient to slowly learn the semantic features of the videos into the model, which requires many weight updates. Inspired by recent success in prototypical learning~\cite{snell2017prototypical, jin2022prototypical}, we use a prototypical module to store the embeddings. Prototypical Networks rely on the idea that there exists an embedding space in which semantically related videos cluster around a single prototype representation.
Given a video $v_i$, the prototypical encoder matches its video representation $\mathbf{v}_j$ with each prototype $\mathbf{p}_j \in P$ according to some distance function $d(\cdot, \cdot): \mathbb{R}^{D} \times \mathbb{R}^{D} \rightarrow \mathbb{R}$, then produces a distribution over $P$ $\mathbb{P}(\mathbf{p}_j \mid v_i)$

\begin{equation}
\mathbb{P}(\mathbf{p}_j \mid v_i) = \frac{\exp (-d(\mathbf{p}_{j}, \mathbf{v}_i))}{\sum_{j'} \exp (-d(\mathbf{p}_{j'}, \mathbf{v}_i))}
\label{eq:prototype_weights}
\end{equation}
\begin{equation}
\mathbf{\tilde{v}}_i
= \sum_{j=1}^{|P|} \underbrace{ \mathbb{P}(\mathbf{p}_j \mid v_i)}_{\substack{\text{Prototype}\\ \text{Importance}}} \mathbf{v}_i
\label{eq:prototype_new_embed}
\end{equation}

where $d(\cdot, \cdot): \mathbb{R}^{D} \times \mathbb{R}^{D} \rightarrow \mathbb{R}$ is a . Here we use the Euclidean distance for $d(\cdot, \cdot)$.

==> src/bak_0527_tab-performance.tex <==
\begin{table*}
\centering
\caption{Performances of \model\ and 7 competitors for warm-start videos. Values in \textbf{bold} and underline represent the best and 2nd best performance in each column, respectively. ``Impr'' denotes the performance improvement of \model compared to the best baseline. % \srijan{very confusing. This table says it is for warm start videos. So what is Head and Tail?}
}\label{tab:warm}
\vspace{-0.2cm}
\textbf{(a) Large Dataset}
\begin{tabular}{l|ccccc|ccccc} 
\toprule
 &  &  \multicolumn{3}{c}{Popular Communities}  &  &  &  \multicolumn{3}{c}{Non-Popular Communities} &  \\ 
\cline{3-5}\cline{8-10}
 & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR \\ 
\midrule
MF & 0.5216 & 0.7194 & 0.6002 & 0.8469 & 0.4734 & 0.1346 & 0.2205 & 0.1820 & 0.3595 & 0.1513 \\
NGCF & 0.5291 & 0.7307 & 0.5597 & 0.8477 & 0.5246 & 0.1399 & 0.2213 & 0.1845 & 0.3680 & 0.1581 \\
LightGCN & 0.5468 & 0.7349 & 0.5675 & 0.8505 & 0.5215 & 0.1537 & 0.2426 & 0.1987 & 0.3832 & 0.1691 \\
SVD-GCN & 0.5677 & 0.7572 & 0.6002 & 0.8514 & 0.5379 & 0.1609 & 0.2539 & 0.2065 & 0.3960 & 0.1739 \\
TiSASRec & 0.5696 & 0.7593 & 0.6029 & 0.8534 & 0.5354 & 0.1668 & 0.2586 & 0.2078 & 0.3956 & 0.1770 \\
TGAT & 0.5679 & 0.7603 & 0.6130 & 0.8530 & 0.5354 & 0.1684 & 0.2590 & 0.2121 & 0.3969 & 0.1775 \\
TGN & \ul{0.5723} & \ul{0.7604} & \ul{0.6140} & \ul{0.8569} & \ul{0.5576} & \ul{0.1687} & \ul{0.2596} & \ul{0.2138} & \ul{0.3970} & \ul{0.1818} \\
\midrule
\textbf{\model} & \textbf{0.6013} & \textbf{0.7816} & \textbf{0.6383} & \textbf{0.8793} & \textbf{0.5822} & \textbf{0.1798} & \textbf{0.2741} & \textbf{0.2263} & \textbf{0.4182} & \textbf{0.1923} \\
\textbf{Impr} & \textbf{5.1\%} & \textbf{2.8\%} & \textbf{4.0\%} & \textbf{3.0\%} & \textbf{4.4\%} & \textbf{6.6\%} & \textbf{5.6\%} & \textbf{5.9\%} & \textbf{5.3\%} & \textbf{5.8\%} \\
\bottomrule
\end{tabular}
\textbf{} \\
\textbf{(b) Small Dataset}\\
\centering
\begin{tabular}{l|ccccc|ccccc} 
\toprule
 & \multicolumn{1}{l}{} & \multicolumn{3}{c}{Popular Communities}  & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{Non-Popular Communities}  & \multicolumn{1}{l}{} \\ 
\cline{3-5}\cline{8-10}
 & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR \\ 
\midrule
MF & 0.3594 0.5211 & 0.4017 & 0.6585 & 0.3356 & 0.0764 & 0.1203 & 0.0991 & 0.1958 & 0.0803 \\
NGCF & 0.3641 & 0.5282 & 0.4100 & 0.6620 & 0.3411 & 0.0807 & 0.1250 & 0.1000 & 0.1816 & 0.0887 \\
LightGCN & 0.3789 & 0.5493 & 0.4167 & 0.6796 & 0.3448 & 0.0852 & 0.1321 & 0.1172 & 0.2241 & 0.0967 \\
SVD-GCN & 0.3893 & 0.5634 & 0.4235 & 0.6839 & 0.3621 & 0.0947 & 0.1415 & 0.1204 & 0.2311 & 0.1011 \\
TiSASRec & 0.3907 & 0.5617 & 0.4287 & 0.6840 & 0.3642 & 0.0948 & 0.1439 & 0.1233 & 0.2335 & 0.1061 \\
TGAT & 0.3922 & 0.5669 & 0.4276 & 0.6845 & 0.3676 & 0.0953 & 0.1445 & 0.1256 & 0.2321 & 0.1095 \\
TGN & \ul{0.4037} & \ul{0.5728} & \ul{0.4324} & \ul{0.6849} & \ul{0.3753} & \ul{0.0981} & \ul{0.1462} & \ul{0.1302} & \ul{0.2358} & \ul{0.1156} \\
\midrule
\textbf{\model} & \textbf{0.4377} & \textbf{0.6092} & \textbf{0.4613} & \textbf{0.7031} & \textbf{0.4026} & \textbf{0.1115} & \textbf{0.1533} & \textbf{0.1428} & \textbf{0.2524} & \textbf{0.1380} \\
\textbf{Impr.} & \textbf{8.4\%} & \textbf{6.3\%} & \textbf{6.7\%} & \textbf{2.7\%} & \textbf{7.3\%} & \textbf{13.6\%} & \textbf{4.8\%} & \textbf{9.7\%} & \textbf{7.0\%} & \textbf{19.4\%} \\
\bottomrule
\end{tabular}
\begin{tabular}{l|cccccccccc}
\toprule
MF & 35.92 $\pm$ 0.30 & 52.21 $\pm$ 0.48 & 40.25 $\pm$ 0.79 & 65.83 $\pm$ 0.52 & 33.47 $\pm$ 0.61 & 7.71 $\pm$ 0.31 & 12.00 $\pm$ 0.33 & 9.93 $\pm$ 1.08 & 19.61 $\pm$ 0.46 & 8.08 $\pm$ 0.24\\
NGCF & 36.39 $\pm$ 0.56 & 53.01 $\pm$ 0.41 & 40.91 $\pm$ 0.25 & 66.30 $\pm$ 0.66 & 34.12 $\pm$ 0.31 & 8.14 $\pm$ 0.07 & 12.52 $\pm$ 0.18 & 10.09 $\pm$ 0.13 & 18.21 $\pm$ 0.11 & 9.09 $\pm$ 0.35\\
LightGCN & 37.95 $\pm$ 0.53 & 55.05 $\pm$ 0.52 & 41.77 $\pm$ 0.36 & 68.21 $\pm$ 0.61 & 34.71 $\pm$ 0.38 & 8.58 $\pm$ 0.23 & 13.16 $\pm$ 0.22 & 11.96 $\pm$ 0.21 & 22.56 $\pm$ 0.31 & 9.74 $\pm$ 0.20\\
SVD-GCN & 38.89 $\pm$ 0.33 & 56.50 $\pm$ 0.37 & 42.45 $\pm$ 0.24 & 68.48 $\pm$ 0.37 & 36.22 $\pm$ 0.29 & 9.50 $\pm$ 0.17 & 14.17 $\pm$ 0.11 & 12.05 $\pm$ 0.13 & 23.16 $\pm$ 0.32 & 10.20 $\pm$ 0.17\\
TiSASRec & 39.17 $\pm$ 0.50 & 56.34 $\pm$ 0.50 & 42.95 $\pm$ 0.39 & 68.39 $\pm$ 0.33 & 36.55 $\pm$ 0.46 & 9.65 $\pm$ 0.22 & 14.38 $\pm$ 0.23 & 12.37 $\pm$ 0.31 & 23.51 $\pm$ 0.31 & 10.60 $\pm$ 0.15\\
TGAT & 39.22 $\pm$ 0.46 & 56.79 $\pm$ 0.17 & 42.65 $\pm$ 0.16 & 68.53 $\pm$ 0.31 & 36.75 $\pm$ 0.29 & 9.64 $\pm$ 0.17 & 14.47 $\pm$ 0.18 & 12.61 $\pm$ 0.32 & 23.27 $\pm$ 0.20 & 11.11 $\pm$ 0.20\\
TGN & 40.33 $\pm$ 0.22 & 57.33 $\pm$ 0.30 & 43.27 $\pm$ 0.25 & 68.60 $\pm$ 0.20 & 37.45 $\pm$ 0.30 & 9.87 $\pm$ 0.03 & 14.58 $\pm$ 0.12 & 12.98 $\pm$ 0.08 & 23.63 $\pm$ 0.10 & 11.57 $\pm$ 0.16\\
INPAC & 43.81 $\pm$ 0.29 & 60.89 $\pm$ 0.40 & 46.11 $\pm$ 0.26 & 70.31 $\pm$ 0.59 & 40.24 $\pm$ 0.44 & 11.14 $\pm$ 0.18 & 15.31 $\pm$ 0.17 & 14.25 $\pm$ 0.31 & 25.28 $\pm$ 0.44 & 13.75 $\pm$ 0.21\\
Impr. & 8.6\% & 6.2\% & 6.6\% & 5.1\% & 7.5\% & 12.9\% & 5.0\% & 9.8\% & 7.0\% & 18.8\%
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Performances of \model\ and 7 competitors for cold-start videos. 
% \yc{I wonder how graph-based recommendations that do not consider temporal aspects can provide not-that-bad inductive reasoning.} \yq{The interaction is not very sparse in our case, so matrix-factorization-based methods can work relatively well.}
}\label{tab:cold}
\vspace{-0.2cm}
\textbf{(a) Large Dataset}
\begin{tabular}{l|ccccc|ccccc} 
\toprule
 &  &  \multicolumn{3}{c}{Popular Communities}   &  &  &  \multicolumn{3}{c}{Non-Popular Communities}   &  \\ 
\cline{3-5}\cline{8-10}
 & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR \\ 
\midrule
MF & 0.5291 & 0.7361 & 0.5669 & 0.8411 & 0.4824 & 0.1069 & 0.1593 & 0.1390 & 0.2600 & 0.1245 \\
NGCF & 0.5632 & 0.7485 & 0.5862 & 0.8380 & 0.5118 & 0.1371 & 0.2285 & 0.1834 & 0.3732 & 0.1508 \\
LightGCN & 0.5768 & 0.7534 & 0.6005 & 0.8373 & 0.5247 & 0.1426 & 0.2515 & 0.1942 & 0.3926 & 0.1576 \\
SVD-GCN & 0.5808 & 0.7633 & 0.6033 & 0.8398 & 0.5344 & 0.1484 & 0.2532 & 0.1944 & 0.3972 & 0.1696 \\
TiSASRec & 0.5853 & 0.7604 & 0.6023 & 0.8380 & 0.5326 & 0.1516 & 0.2538 & 0.1990 & 0.3973 & 0.1705 \\
TGAT & \ul{0.5896} & \ul{0.7638} & 0.\ul{6104} & 0.\ul{8435} & \ul{0.5497} & 0.1586 & 0.2549 & 0.2067 & 0.4009 & \ul{0.1760} \\
TGN & 0.5872 & 0.7636 & 0.6102 & 0.8404 & 0.5452 & \ul{0.1623} & \ul{0.2552} & \ul{0.2080} & \ul{0.4019} & 0.1732 \\
\midrule
\textbf{\model} & \textbf{0.6174} & \textbf{0.7855} & \textbf{0.6397} & \textbf{0.8677} & \textbf{0.5776} & \textbf{0.1764} & \textbf{0.2705} & \textbf{0.2205} & \textbf{0.4238} & \textbf{0.1873} \\
\textbf{Impr.} & \textbf{4.7\%} & \textbf{2.8\%} & \textbf{4.8\%} & \textbf{2.9\%} & \textbf{5.1\%} & \textbf{8.6\%} & \textbf{6.0\%} & \textbf{6.0\%} & \textbf{5.5\%} & \textbf{6.4\%} \\
\bottomrule
\end{tabular}

\textbf{} \\
\textbf{(b) Small Dataset}\\
\begin{tabular}{l|ccccc|ccccc} 
\toprule
 &  &  \multicolumn{3}{c}{Popular Communities}  &  &  &  \multicolumn{3}{c}{Non-Popular Communities}   &  \\ 
\cline{3-5}\cline{8-10}
 & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR & NDCG@5 & Rec@5 & NDCG@10 & Rec@10 & MRR \\ 
\midrule
MF & 0.3524 & 0.5785 & 0.4167 & 0.8508 & 0.2922 & 0.0730 & 0.1134 & 0.1077 & 0.2150 & 0.0961 \\
NGCF & 0.3631 & 0.5864 & 0.4332 & 0.8351 & 0.3194 & 0.0816 & 0.1237 & 0.1099 & 0.2320 & 0.0991 \\
LightGCN & 0.3958 & 0.5890 & 0.4421 & 0.8639 & 0.3221 & 0.0825 & 0.1289 & 0.1107 & 0.2262 & 0.0984 \\
SVD-GCN & 0.4034 & 0.6073 & 0.4515 & 0.8743 & 0.3283 & 0.0800 & 0.1289 & 0.1136 & 0.2268 & 0.1011 \\
TiSASRec & 0.4172 & 0.6466 & 0.4682 & 0.8807 & 0.3643 & 0.0849 & 0.1366 & 0.1142 & 0.2320 & 0.1071 \\
TGAT & 0.4244 & 0.6709 & 0.4779 & 0.8814 & 0.3664 & 0.0839 & 0.1392 & 0.1149 & 0.2371 & 0.1073 \\
TGN & \ul{0.4273} & \ul{0.6753} & \ul{0.4797} & \ul{0.8831} & \ul{0.3696} & \ul{0.0883} & \ul{0.1443} & \ul{0.1157} & \ul{0.2396} & \ul{0.1094} \\
\midrule
\textbf{\model} & \textbf{0.4646} & \textbf{0.7155} & \textbf{0.5083} & \textbf{0.9110} & \textbf{0.3847} & \textbf{0.1008} & \textbf{0.1526} & \textbf{0.1272} & \textbf{0.2506} & \textbf{0.1180} \\
\textbf{Impr.} & \textbf{8.7\%} & \textbf{5.9\%} & \textbf{5.9\%} & \textbf{3.1\%} & \textbf{4.1\%} & \textbf{14.2\%} & \textbf{5.8\%} & \textbf{10.0\%} & \textbf{4.6\%} & \textbf{7.9\%} \\
\bottomrule
\end{tabular}
\end{table*}

==> src/bak_intro_0201_8pm.tex <==
\section{Introduction}\label{sec:intro}

\srijan{
Background: 
1. Users aggregate around topical interest communities. Common on reddit, whatsapp groups, telegraph groups. Users consume and share information on these communities. Prior research has shown that communities interact with one other. 
2. Information flows across these communities. Information is multimodal (image, video). Information has varying veracity, some information is bad. 
3. Community Information Pathway Prediction (CIPP) is thus important. If we can predict the communities where information will appear, this can be beneficial in many use cases. For bad information, it can be used for intervention; for marketers, this can be used for better visibility and reach. 

Challenges:
1. This is hard because community-community influence is not known.
2. information flow is complex and multimodal (image, text, video). Users interact with communities over time. This creates a dynamic graph. 
3. information ecosystem is changing over time with new content and new communities. 

Contributions:
1. collect data, and analyze sharing behavior to identify distinct sharing patterns. 
2. use this to infer community-community influence graphs (CCIGs) that estimates the influence 
3. Create a dynamic graph framework that is built on the CCIG. The framework learns from the multimodal data and the dynamics of the interactions between users and communities. 
4. Validation: experiments are conducted. better results than baselines. 
}

\vspace{1mm}
\noindent{\bf Background.}
% The proliferation of various forms of content, including news articles, viral videos, and online rumors, significantly impacts our perceptions and comprehension of the world. 
% \yc{Can we provide various examples of information diffusion in the real world? Also, we can add a figure that shows there are a lot of scenarios of information diffusion so that our research motivation can be highlighted.}
% \yiq{% Some examples of information diffusion on social media: 1) News articles shared on LinkedIn: News articles that are relevant to a particular industry or profession spread quickly on LinkedIn, as users share them with their professional networks. 2) Viral videos on YouTube that contain misinformation or political bias are shared by many users on Reddit, causing it to spread rapidly among the social network's users. }
% \srijan{You need to make a case that users join communities, commumnities exert influence on each other, which can help in influence pathway prediction.}

\srijan{Talk about how users join communities of their interest to consume and share information within those communities. large communities become hubs of information.}
Social media has transformed the way information is spread online, allowing users to communicate with each other and share contents on various online communities (\eg, Twitter and Reddit). 
With the fast-evolving social media, such a spread of information appears rapidly and coveys various forms of contents, including news articles, viral videos, and online rumors. 
In particular, we see that content, including
misinformation, hate speech, or political bias, tend to be easy to spread~\cite{shu2019defend, shu2017fake, wang2018eann}. 
\srijan{talk about how such harmful content spreads from one community to another. thus it is important to understand the influence that communities have on one another.}
% For instance, videos on YouTube that contain \yc{can we provide a concrete example of the spread of YouTube videos having misinformation on Reddit based on the authorized source?} 
\hide{Such spread of information can have adverse real-world impact. In 2016, a YouTube video claiming that a Washington D.C. pizza restaurant was connected to a child trafficking ring was posted and shared on Twitter and Reddit~\cite{aisch2016dissecting, gillin2016pizzagate}. Despite its fast debunk, the misinformation spread rapidly on both platforms, leading to real-world consequences when a man fired a rifle inside the restaurant. This incident highlights the dangers of misinformation spread through social media and the importance of verifying information before sharing it.}

% This has led to the rapid spread of various forms of information, including news articles, viral videos, and online rumors. 

% for various fields such as online recommendation, advertising and public opinion formation. 
% For online recommendation and advertising, uncovering the information pathways can help us identify suitable online communities so that users can spontaneously spread the content across different online communities. 

For this reason, there has been a marked increase in research initiatives aimed at comprehending the information spread on various social media platforms from different perspectives, such as the impact of misinformation~\cite{jin2022towards, yang2022reinforcement}, the effect of social media on individual and collective behavior~\cite{shareef2020group, zhou2012social}, and the analysis of information diffusion from an algorithmic perspective~\cite{myers2012information, yang2010modeling}.  
% and predictions of information pathways [cites].
Among these, the problem of {\bf Information Pathway Prediction (IPP)} has gained particular attention in recent years due to its wide-ranging practical applications~\cite{li2021capturing, feng2022h, gomez2013structure}. 
Previous research have shown that while the information spreading appears to be random, the underlying pathways over which information propagates remain relatively stable~\cite{gomez2012inferring, qiu2018deepinf}. 
% These pathways can be thought of as upstream and downstream connections. 
% \yc{the meanings of upstream and downstream are vague, so I removed this sentence.}
Their stability is partially due to the behavior of common users who repeatedly spread information through the same channels, creating a reinforcement of the underlying information pathways. 
% As a result, it becomes easier for misinformation to spread through these stable pathways, making it important to understand and monitor these pathways to help prevent the spread of misinformation.
Furthermore, recent works have focused on investigating the information propagation between individual users, \ie, ``microscopic'' influence, and predicting information pathways on the user-user level~\cite{chen2022ctl, zhou2020variational, li2017deepcas, myers2014bursty}. 
For example, Qiu et al.~\cite{qiu2018deepinf} predicts a user's action status based on her nearest neighbors and local structural information, while Wu et al.~\cite{wu2020diffnet++} models the user-level interest/influence diffusion for improved social recommendations. 
% \yc{Describe briefly a representative previous work that focuses on user-level?}
\srijan{you need to compress the above findings and talk also about community-level influence. Talk about findings from papers by me, Ashton Anderson, Chenhao Tan.}

Effective solutions to the IPP problem can bring significant benefits to various organizations and individuals.
% Understanding these information pathways is of vital importance and has a wide range of practical applications.
In online marketing, businesses can launch more successful marketing campaigns by 
% understanding the cross-community information flow and 
identifying key influencers [cite]. 
In combating misinformation, online moderators can better identify vulnerable individuals susceptible to certain false information~\cite{gomez2013structure, ng2022cross}. 
% can be inferred by analyzing the content of the misinformation.
% \yc{We will claim that we are the first to investigate the community-community influence pathways, so I removed community-related sentences here. It would be better to provide these as our work's implications.}

% In online marketing, by understanding the mechanisms of information flows across different communities, businesses can more effectively target key influencers in their marketing campaigns. For misinformation mitigation, we are able to infer vulnerable communities subject to certain misleading information given the content of misinformation. In this sense, many methods have been proposed to study such information spread~\cite{gomez2013structure, ng2022cross}.



% However, predicting the pathway of online information dissemination is a challenging task due to the complex and dynamic nature of the diffusion environment. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Challenges
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \yc{C2: static and dynamic features => need to design a joint modeling}
% \yc{C3: no data => need to collect new dataset}
\vspace{1mm}
\noindent{\bf Challenges.}
The aforementioned works made important steps in accurately predicting information pathways between individual users.
However, in this work, we explore non-trivial challenges of the IPP problem: {\bf(C1) Macroscopic Influence}; {\bf(C2) Complex Diffusion Environment}; {\bf(C3) Inductive Nature}. 
% predicting online information pathways poses unique challenges.
% (mixture of different contents, users, platforms) => need to focus on a specific type of content on a specific platform first

\begin{table*}
\centering
\caption{Examples of cross-community information flow in our datasets. It demonstrates that a video is usually shared on a set of semantically similar subreddits. \srijan{is this sequential sharing? if so, use arrows to show the sequence.}}
\vspace{-0.2cm}
\label{tab:subredditsSharingVideo}
\begin{tabular}{c|c} 
\toprule
\toprule
\textbf{Title of the Video} & \textbf{Subreddits Sharing the Video}  \\ 
\midrule
Canadian Trudeau Investigation & \begin{tabular}[c]{@{}c@{}}Liberate\_Canada, conspiracy, TheNewRight, \\PeoplesPartyofCanada, Canada\_First\end{tabular} \\ 
\hline
Reviews: Super Dragon Ball Heroes Episode 19 & \begin{tabular}[c]{@{}c@{}}promote, AnimeReviews, anime\_manga,\\YouTubeAnimeCommunity, Anime\_and\_Manga\end{tabular} \\ 
\hline
Warcraft 3 Reforged Cutscene Only & WC3, pcgaming, warcraft3, gaming, legaladviceofftopic \\ 
\hline
Practical Greeting Phrases for Chinese New Year & learnchinese, learnmandarin, learnmandarinchinese \\ 
\hline
Accepting what is. (Realize Instant Freedom) & \begin{tabular}[c]{@{}c@{}}AnxietyDepression, Soulnexus,~SpiritualAwakening,\\Meditation, spirituality, awakened, inspiration\end{tabular} \\ 
\hline
Covid-19 Explained with Data Science & \begin{tabular}[c]{@{}c@{}}Python, CoronavirusUS, CanadaCoronavirus,\\CoronaVirus\_2019\_nCoV, CoronavirusUK\end{tabular} \\ 
\hline
\multicolumn{1}{l|}{Implement RNN-LSTM for Music Genre Classification} & learnmachinelearning, Python, tensorflow, musictheory \\
\bottomrule
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table*}

Regarding (C1), the macroscopic influence (i.e., community-to-community influence) is critical for understanding how information spreads, as different communities may have different norms, values, and communication patterns that influence the temporal and geometric patterns of information diffusion [cites].
% Thus, it is important to understand the mechanisms of information flows across different communities. 
However, as we mentioned above, most existing works usually focus on predicting information pathways at the user level (\ie, microscopic influence) [cites]. 
Furthermore, existing datasets [cites], which are used for the IPP problem, only contain limited information about community structures, making it difficult to study cross-community information spread. 

Regarding (C2), the spread of information is characterized by a complex and dynamic diffusion environment. 
The diffusion speed of different types of contents can vary significantly. 
For example, news stories tend to propagate quickly, rather than other types of content \red{(\eg, )}.
% , while  may spread more slowly or in specific patterns.
Additionally, some contents may only be shared within specific and limited communities, such as those related to a shared ethnicity or geographic location, while others may create far-reaching cascades and reach multiple and disparate communities. 
Therefore, it is important to understand these complexities for accurately predicting the spread of online information.

% Secondly, pathway prediction in cold-start scenarios present additional challenges. The absence of historical data makes it harder to predict which communities are most likely to share the content, and how quickly it will spread. Cold-start scenarios can be particularly challenging in the context of online information dissemination, as new pieces of content are constantly being created and shared. 


Regarding (C3), the network over which information propagations take place is usually unknown and unobserved~\cite{gomez2012inferring, rong2016model}.
% it is non-trivial to identify a way to successfully trace the contagion.  
In particular, as the network evolves over time, new contents can be propagated to new communities.
In this case, we only observe where new content is propagated to the new communities and when it takes place. 
The underlying community influence, \ie, who influences the propagation, remains unknown.
Therefore, the IPP problem in cold-start scenarios can be challenging, as the absence of historical data makes it harder to predict which communities are most likely to share the content, and how quickly it will spread. 




\vspace{1mm}
\noindent{\bf Our Work.}
In this work, we aim to \ul{investigate the dynamics of cross-community information flow while jointly addressing the challenges of complex diffusion environment, macroscopic influence, and inductive nature}.
Towards this goal, we collect relevant datasets that can simulate community-community information pathways, and develop a novel framework \textbf{\model} that predicts {\bf\underline{In}}formation {\bf\underline{P}}athway {\bf\underline{A}}cross Online {\bf\underline{C}}ommunities. 

\yq{
From Ajay: First contribution: 
we have a key finding: time interval, consistency across sharing events. 
Propose a new measure of influence. which help us discover hidden relations among online communities
Based on this, we design a new frame work \model that characterizes macroscopic influence
\model, which is a graph representation of macroscopic influence.
% allow us to represent the data in a graph structure
validation: collect the data, perform extensive experiments
}

To address (C1), we focus on the spread of visual contents on social media, which clearly reveals information diffusion at the community level.
To this end, we collect two large-scale datasets, which include massive visual contents on YouTube and long-term community activity on Reddit. This allow us to identify the patterns and factors that drive the diffusion of online visual content.
% the diffusion of YouTube videos on Reddit.
Note that Reddit is ideal for studying cross-community information diffusion since it provides numerous communities, named ``subreddits,'' that are dedicated to specific topics or interests. 
% Such community structures make it easy to identify and track information that is spread among these communities. 
% Furthermore, Reddit's user base is diverse and representative of a wide range of interests, making it a valuable resource for studying information diffusion across different communities.

Then, we design \model\ while modeling cross-community information flow under our datasets (\eg, Tab.~\ref{tab:subredditsSharingVideo}). 
Specifically, we leverage the structural information as manifested in the content sharing events of online communities. 
By doing so, we can capture correlations between visual contents and communities and address the rapid shifts of information diffusion, thereby successfully addressing (C2). 

Moreover, \model\ is based on the observation that users exhibit similar temporal patterns in their content sharing behavior. This allows us to utilize the time intervals between consecutive shares as a powerful indicator of influence. This simple yet powerful method enables us to characterize the relationships of influence among communities and infer the most likely communities to share a video with limited information.
Thus, we provide excellent inductive capabilities on unknown contents (\ie, (C3)).


% By doing so, we can thoroughly understand the patterns and factors that drive the diffusion of online visual content.

% Reddit, with its subcommunities of users organized around specific topics, offers a unique and rich environment to study the spread of information. By analyzing how YouTube videos are shared and discussed within these subcommunities, we aim to gain insights into the patterns and factors that drive the diffusion of online visual content. 

% In this paper, we aim to study this problem and propose a method that addresses the unique challenges that arise in predicting the spread of online information. Specifically, we focus on the importance of community structure and the impact of cold-start scenarios on the prediction of information pathways. Furthermore, we propose a new dataset that specifically focuses on identifying community structure and measuring community influence.

% \yc{describe our conceptual idea to address the challenges above.}

\vspace{1mm}
\noindent{\bf Contributions.}
Our main contributions are as follows:
\begin{itemize}[leftmargin=*]
    % Our datasets cover a wide range of features, such as the textual and graph-structural information of online posts and videos.
    
    \item \textbf{Novel Multi-modal Datasets}: % We collect data with sufficient microscopic level information
    To comprehensively study IPP, we collect two large-scale and multi-modal datasets that enable us to simulate the diffusion of visual contents at the community level for information pathway prediction.
    % Our datasets specifically focus on identifying community structure and measuring community influence. 
    Our datasets can provide valuable insights into how information spreads within and across different communities. % and can help to improve the accuracy of predictions in this area.

    \item \textbf{Effective Prediction Framework}: We propose \model, a novel information pathway prediction framework that bridges the static content and community attributes with the dynamic nature of information propagation. 
    % To the best of our knowledge, our framework offers the novel capability to characterize macroscopic influence for the first time.
    
    % learns the dynamics of cross-community information flow.
    % Instantiate the CTDG with the new static representation, richer IPP model
    % that jointly and efficiently learns static and dynamic features regarding the diffusion of online visual contents on social media platforms.
    % To the best of our knowledge, we are the first to investigate the community-community influence pathways (\ie, macroscopic influence).
    % computationally efficient graph-based framework for modeling online information pathways.
    \item \textbf{Comprehensive Evaluation}: We demonstrate the effectiveness of \model framework and its design choices through extensive experiments in various scenarios, \eg, prediction of cold/warm-start videos on communities with various activity levels.
    % \yc{Highlight the accuracy improvement or key findings.}
    
\end{itemize}

Our code is available at Anonymous GitHub\footnote{\url{https://anonymous.4open.science/r/KDD2023-F803/}}. 
We plan to release all the datasets and code upon the acceptance of this work. 





==> src/reserved-for-tkde.tex <==
\section{(RESERVED FOR TKDE)}

\subsection{Metrics}

For each positive video-community interaction, we followed the common strategy~\cite{he2017neural, elkahky2015multi, koren2008factorization} to randomly sample 100 items that are not interacted by the user, ranking the test item among the 101 items. Therefore, there is only 1 relevant result for each interaction.

\textbf{NDCG@K} is a measure of the model's ranking quality, defined as:

\begin{equation}
\text{NDCG@K} = \frac{\text{DCG@K}}{\text{IDCG@K}},
\end{equation}
where DCG@K is the Discounted Cumulative Gain at K that measures the relevance values of all results in a ranked list.

\begin{equation}
\text{DCG@K} = \sum_i \frac{rel_i}{\log_2(i + 1)},
\end{equation}
where $rel_i$ is the relevance of the community at position $i, i \in [1, K]$. Since the test community is the only relevant one in this scenario, $rel_i$ = 1 if the test community is at position $i$ and 0 otherwise. The Ideal DCG@K (IDCG@K) is the maximum possible DCG@K given the ground truth, which is 1. If the test community is not in the top-K results, then NDCG@K = 0.


\textbf{Recall@K} measures the number of relevant items were returned against how many relevant items exist in the entire dataset.


\textbf{Mean Reciprocal Rank (MRR)} measures the average of the reciprocal ranks of the first relevant community (positive user-community interaction) in the ranked list. The reciprocal rank is the multiplicative inverse of the rank of the test community in the ranked list, \ie, $\text{RR} = 1 / r_{test}$,
% \begin{equation}
% \text{RR} = 1 / r_{test},
% \end{equation}
where $\text{RR}$ is the reciprocal rank, and $r_{test}$ is the rank of the test community. If the test community is not in the ranked list, the reciprocal rank is 0.
The MRR is computed by averaging the reciprocal ranks:

\begin{equation}
MRR = \sum_{v \in V} \frac{RR}{|V|}.
\end{equation}
MRR focuses on the rank of the first relevant community, which is particularly useful in scenarios where we are only concerned the top-ranked communities. MRR ranges from 0 to 1, with higher values indicating better performances.



\subsection{Results on the Misinformation Datasets}

\begin{table*}
\centering
\caption{Results}
\label{tab:dataset_stats}
\begin{tabular}{l|ccccc}
\toprule
\textbf{ } & \textbf{ NDCG@5 } & \textbf{ Rec@5 } & \textbf{ NDCG@10 } & \textbf{ Rec@10 } & \textbf{ MRR }\\
\hline
TiSASRec & 0.6454 $\pm$ 0.0133 & 0.7474 $\pm$ 0.0083 & 0.6525 $\pm$ 0.0057 & 0.7853 $\pm$ 0.0133 & 0.6081 $\pm$ 0.0102\\
TGAT & 0.6728 $\pm$ 0.0102 & 0.7805 $\pm$ 0.0151 & 0.6805 $\pm$ 0.0086 & 0.8175 $\pm$ 0.0133 & 0.6266 $\pm$ 0.0074\\
TGN & 0.6752 $\pm$ 0.0053 & 0.7816 $\pm$ 0.0049 & 0.6818  $\pm$ 0.0041 & 0.8235 $\pm$ 0.0133 & 0.6346 $\pm$ 0.0058\\
INPAC & 0.7127 $\pm$ 0.0066 & 0.8260 $\pm$ 0.0025 & 0.7286 $\pm$ 0.0048 & 0.8750 $\pm$ 0.0133 & 0.6854 $\pm$ 0.0042\\
\midrule
Impr. & 5.5\% & 5.7\% & 6.9\% & 6.2\% & 8.0\% \\
 \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
  \begin{tabular}{l|ccccc} \\
  & NDCG@5 & Rec@5  & NDCG@10& Rec@10 & MRR    \\
  \toprule
  TiSASRec & 0.7026 $\pm$ 0.0128 & 0.8580 $\pm$ 0.0128 & 0.7261 $\pm$ 0.0128 & 0.8846 $\pm$ 0.0078 & 0.6604 $\pm$ 0.0128 \\
  TGAT     & 0.7226 $\pm$ 0.0072 & 0.8526 $\pm$ 0.0022 & 0.7407 $\pm$ 0.0066 & 0.9017 $\pm$ 0.0044 & 0.6758 $\pm$ 0.0111 \\
  TGN      & 0.7230 $\pm$ 0.0038 & 0.8589 $\pm$ 0.0100 & 0.7416 $\pm$ 0.0108 & 0.9039 $\pm$ 0.0073 & 0.6803 $\pm$ 0.0034 \\
  \model    & 0.7727 $\pm$ 0.0057 & 0.9050 $\pm$ 0.0065 & 0.7855 $\pm$ 0.0085 & 0.9458 $\pm$ 0.0033 & 0.7356 $\pm$ 0.0058 \\
  \midrule
  Impr.    & 6.9\%   & 5.4\%   & 6.0\%    & 4.6\%   & 8.1\% \\
  \bottomrule
\end{tabular}
\end{table*}

We show the results on the two datasets about misinformation. The \textbf{Misinfo-L} dataset contains 275,629 misinformative links shared on 14,991 communities over a 5-year period (January 2018 - December 2022). The \textbf{Misinfo-S} dataset contains 20,211 misinformative links shared on 1,919 communities over a 3-month period (January 2020 - March 2020). The statistics of the datasets are shown in Table~\ref{tab:data}. 

\subsection{Validation of CIG}

The primary objective of this experiment is to authenticate the quality of our dataset and evaluate if a model trained on this data can discern significant inter-community relations. To this end, we employed three human annotators to assess the CIG for 200 videos, generated through three distinct methods.
% We conduct human experiments to evaluate the validity of resulting CIGs. The goal is to verify the quality of our dataset and see if a model trained on the data can learn meaningful community-community relationships. To this end, we enlisted the help of three human annotators to evaluate the CIG for 200 videos generated using three different methods.

\begin{itemize}[leftmargin=*]
    \item \model constructs the CIG using our proposed algorithm;
    \item \model-Seq constructs the CIG using the \model-Seq method as discussed in the ablation studies (Section 4.3). 
    % It connects the community nodes sequentially, i.e., we create a directed edge from $s_j$ to $s_k$ if they are adjacent in the corresponding propagation sequence;
    \item ER employs the Erdos-Renyi graph~\cite{erdos2011evolution} to construct the CIG while maintaining the graph's density. Specifically, we calculate the probability of edge connection using $\frac{|E|}{|N||N-1|}$, where $|N|$ and $|E|$ represent the number of nodes and edges in the original graph, respectively.
\end{itemize}

For each video, we asked the annotators to manually rank the generated CIGs based on their perceived level of community-community influence, by checking each subreddit involved in the CIG. We also randomly positioned the figures shown to each annotator to ensure that they could not identify the method used solely based on the order of the figures.
After the experiment, we asked the annotators to go through the plots again with the method name visible. The goal is to let them provide feedback about the generated plots.

Our evaluation results indicate that, on average, the CIGs generated using \model, \model-Seq, and ER are ranked the best 77.8\%, 18.2\%, and 4.0\% of the time, respectively. This suggests that our proposed algorithm (\model) is the most reasonable under most circumstances. Additionally, we found that the annotators agreed upon 86\% of the rankings.
The annotator said that the CIGs generated random method (ER) usually have community-community edges that are not explainable. For example, for the video ``Americas New Drinking Problem: The Trump Administration Rolls Back the Clean Water Act,'' the annotator reported that the constructed CIG using ER connects the two communities it propagated to ``r/water'' with ``r/Corruption,'' which do not have direct semantic relationships. This indicates that the random method can introduce spurious correlations. The CIGs constructed by \model-Seq is more reasonable, as it sequentially connects ``r/water,'' ``r/Health,'' ``r/Environmental\_Policy,'' ... ``r/GreenParty,'' ``r/Green,'' ``r/activism,'' and so on, which reflects the sharing process (how the video gradually reach a wider audience that are concerned with different topics) the transition of users point of interests.

Among all methods, our proposed method (\model) is the best, as semantically similar subreddits are densely connected to each together. For example, ``r/GreenParty,'' ``r/Green,'' ``r/activism,'' ``r/alltheleft,'' form a clique, whereas subreddits about health and drinking water such as ``r/Health'' and ``r/water'' form a clique.

% Overall, the model trained on the data can learn meaningful community-community relationships, which demonstrates that our datasets contain abundant meaningful posting information for promising models to be learned.



\subsection{Ablation Studies on the Aggregation Scheme}

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.44\textwidth]{fig/VaryAggregationScheme.pdf}
    \includegraphics[width=0.25\textwidth]{fig/VaryAggregationScheme_MRR_NDCG.pdf}
    \includegraphics[width=0.21\textwidth]{fig/VaryAggregationScheme_Rec.pdf}
    \caption{Performances of different aggregation methods for video and channel embeddings on the Large dataset. 
    }
    \label{fig:aggregation}
\end{figure}

In Section~\ref{sec:video}, we aggregated two feature vectors, \ie, video and channel, to obtain the embeddings of videos. To compare the impact of using different aggregation schemes, we made three variants of \model, \ie, \model(Concat), \model(Add), and \model(Mul), each of which uses concatenation, addition, or multiplication as the aggregation schemes.
Figure~\ref{fig:aggregation} shows the results, where $x$-axis indicates the metrics and $y$-axis indicates the performances.
From Figure~\ref{fig:aggregation}, we observe that \model(Mul) outperforms other variants of \model, with the greatest performance improvement on MRR. 
The results also demonstrate that all the variants of \model\ outperform the strongest baseline TGN. 


\subsection{Examples of Model Prediction}

We present 8 videos and their respective top 3 predictions. The first 4 videos have correct predictions, meaning the ground-truth community is within the top 3 predicted communities.

\begin{itemize}
    \item The ``Train'' column displays the communities in which a video was shared during training.
    \item The ``Predicted'' column shows the communities predicted during test time, ordered by their predicted probabilities in descending order. Correct predictions are highlighted in Bold.
    \item The ``Test'' column shows the ground-truth communities during test time.
\end{itemize}


\begin{table*}[t]
\hspace{-1cm}
\centering
\caption{Examples of Correct Predictions by \model}
\label{tab:CorrectPred}
% \begin{tabular}{c|ccc} 
\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}p{0.25\textwidth}|>{\centering\arraybackslash}p{0.33\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}>{\centering\arraybackslash}p{0.18\textwidth}}
\hline
 & Train & Predicted & Test \\ \hline
\multirow{3}{*}{\shortstack{Dancing Israelis and \\ The ``Art Student'' Spy Ring \\ - 9/11 (What Really Happened)}} & \multirow{3}{*}{\shortstack{ConspiracyII,  israelexposed, \\conspiracy}} & \multirow{3}{*}{\shortstack{ FalseFlagWatch, 911, \\ TopConspiracy }} & \multirow{3}{*}{TopConspiracy} \\
 & & & \\
 & & & \\
 \midrule
\multirow{3}{*}{\shortstack{(Black Metal) Rites of Passage \\-Patrizio Lucentini}}  & \multirow{3}{*}{ \shortstack{BandCamp, MusicInTheMaking, mymusic, \\ PlayingGuitar, ratemysong, ratemyband, \\ RedditorMadeMusic, userproduced}} & \multirow{3}{*}{\shortstack{shareyourmusic, Songwriters,\\ ThisIsOurMusic}} & \multirow{3}{*}{shareyourmusic} \\
 & & &  \\
 & & &  \\
\midrule
\multirow{2}{*}{\shortstack{Halogen Mosaic \\ (Original Game Soundtrack) }} & \multirow{2}{*}{newgamemusic, gamemusic} & \multirow{2}{*}{Games, gamemusic\_jp, PS4} & \multirow{2}{*}{gamemusic\_jp} \\
 & & &  \\
 \midrule
\multirow{2}{*}{\shortstack{FULL DAY 1: Senate Impeachment \\ Trial Gets Underway}}  & \multirow{2}{*}{The\_Congress, The\_Donald} & \multirow{2}{*}{\shortstack{AskThe\_Donald, politics, \\Impeach\_Trump}} & \multirow{2}{*}{AskThe\_Donald} \\ 
 & & & \\
\hline
\end{tabularx}
\end{table*}




\begin{table*}[t]
\hspace{-1cm}
\caption{Examples of Incorrect Predictions by \model}
\label{tab:IncorrectPred}
\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}p{0.25\textwidth}|>{\centering\arraybackslash}p{0.3\textwidth}>{\centering\arraybackslash}p{0.2\textwidth}>{\centering\arraybackslash}p{0.2\textwidth}}
\hline
\centering
 & Train & Predicted & Test \\ \hline
\multirow{3}{*}{\shortstack{Is God Immoral Because \\ of the Atrocities Committed \\ in the Old Testament?}} & \multirow{3}{*}{\shortstack{TrueChristian, Christian}} & \multirow{3}{*}{\shortstack{exchristian, Christianity, \\ OpenChristian}} & \multirow{3}{*}{DebateReligion} \\
 & & & \\
 & & & \\
 \midrule
\multirow{3}{*}{\shortstack{Derivation of the \\ Navier-Stokes Equations}}  & \multirow{3}{*}{ \shortstack{StructuralEngineering, \\ LearnEngineering, \\ aerospace}} & \multirow{3}{*}{\shortstack{AerospaceEngineering, \\ MechanicalEngineering, \\ civilengineering}} & \multirow{3}{*}{GetMoreViewsYT} \\
 & & &  \\
 & & &  \\
\midrule
\multirow{2}{*}{\shortstack{Katatonia - Lacquer \\ (from City Burials)}} & \multirow{2}{*}{progmetal, Metal} & \multirow{2}{*}{\shortstack{metalguitar, coversongs, \\ NameThatSong}} & \multirow{2}{*}{doommetal} \\
 & & &  \\
 \midrule
\multirow{2}{*}{\shortstack{Beat Saber VR Gameplay \\ \& First Impressions}}  & \multirow{2}{*}{VRGaming, virtualreality} & \multirow{2}{*}{\shortstack{gamingvids, SteamVR, \\ YouTubeGamers}} & \multirow{2}{*}{oculus} \\ 
 & & & \\
\hline
\end{tabularx}
\end{table*}

From Table~\ref{tab:CorrectPred}, we observe that the predicted communities share commonalities with the video. For instance, the video \textit{``Dancing Israelis and The `Art Student' Spy Ring - 9/11 (What Really Happened)''} discusses a 9/11 conspiracy theory, and our model predicts it to be shared among subreddits about conspiracy, misinformation, and the 9/11 event. From Table~\ref{tab:IncorrectPred}, observe that, in most cases, the predictions are reasonable. For example, the video \textit{``Derivation of the Navier-Stokes Equations''} is predicted to be shared in engineering-related subreddits, although it was actually shared in ``GetMoreViewsYT'' in the test set. The prediction failure can be partly attributed to the random nature of content sharing, as subreddits like ``GetMoreViewsYT'' is a common community for content creators to share their videos.

Similarly, for \textit{``Beat Saber VR Gameplay \& First Impressions,''} a video about VR gaming, the predicted subreddits pertain to VR and gaming, just like the ground-truth data. This indicates that even though the prediction may not exactly match the ground truth, our proposed model can still provide reasonable predictions that closely align with the ground-truth communities.

Overall, the experimental results show that our model can make reasonable predictions by considering the content of the videos and the subreddit-subreddit topical similarities.

